Language Models for Code Optimization: Survey, Challenges and Future Directions

Language models (LMs) built upon deep neural networks (DNNs) have recently demonstrated breakthrough effectiveness in software engineering tasks such as code generation, completion, and repair. This has paved the way for the emergence of LM-based code optimization techniques, which are crucial for enhancing the performance of existing programs, such as accelerating program execution time. However, a comprehensive survey dedicated to this specific application has been lacking. To fill this gap, we present a systematic literature review of over 50 primary studies, identifying emerging trends and addressing 11 specialized questions. Our findings reveal five critical open challenges, such as balancing model complexity with practical usability, cross-language/performance generalizability, and building trust in AI-driven solutions. Furthermore, we provide eight future research directions to facilitate more efficient, robust, and reliable LM-based code optimization. Thereby, this study aims to provide actionable insights and foundational references for both researchers and practitioners in this rapidly evolving field.

==> Tables/RQ_evaluation_metric.tex <==
\begin{table}[t!]
  \caption{The taxonomy of evaluation metrics (one study might be in multiple categories).}
% \vspace{-0.3cm}
\centering
\footnotesize
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lllll}
\toprule
\textbf{Category} & \textbf{Total \#} & \textbf{Evaluation metric} & \textbf{\# studies} & \textbf{Reference} \\ \hline
\multirow{5}{*}{Performance improvement} & \multirow{5}{*}{49} & Percentage performance   improvement (\%PI) & 21 & \cite{DBLP:journals/corr/abs-2310-02304,   DBLP:journals/corr/abs-2408-03408, pan2024ecodemasteringefficientcode,   DBLP:journals/corr/abs-2405-15189, DBLP:conf/nips/ShinnCGNY23,   DBLP:conf/apsec/ShirafujiOSMW23, DBLP:conf/euromlsys/GrubisicSSLMC24,   DBLP:journals/nature/RomeraParedesBNBKDREWFKF24,   DBLP:journals/corr/abs-2401-08500, DBLP:journals/corr/abs-2306-17077,   DBLP:journals/corr/abs-2309-07062,   ishida2024langpropcodeoptimizationframework,   DBLP:journals/corr/abs-2407-14044, DBLP:conf/sigsoft/GargMCSW22,   DBLP:journals/corr/abs-2403-14714, DBLP:journals/corr/abs-2406-12502,   DBLP:journals/corr/abs-2407-02524, choi2024iterative, qu2024dynamic,   DBLP:conf/hpec/GuoM22, li2024instructcoderinstructiontuninglarge} \\ \cline{3-5} 
 &  & Speedup   (SP) & 10 & \cite{gao2024searchbasedllmscodeoptimization,   DBLP:journals/corr/abs-2404-18864, DBLP:journals/corr/abs-2406-04693,   DBLP:journals/corr/abs-2312-05657, DBLP:conf/iclr/ShypulaMZ0GYHNR24,   DBLP:journals/corr/abs-2406-11935, DBLP:journals/corr/abs-2407-14044,   DBLP:journals/pacmpl/YeZSS23, xu2024optimizing, zhang2024codedpo} \\ \cline{3-5} 
 &  & Performance   improvement (PI) & 16 & \cite{yao2024rtlrewritermethodologieslargemodels,   shivashankar2024betterpythonprogrammingall,   DBLP:journals/corr/abs-2406-07496, DBLP:journals/corr/abs-2309-14846,   DBLP:journals/concurrency/HanLDLZ24, hemberg2024evolving, han2024generating,   jain2022jigsaw, palkowski2024gpt, sun2024autosat, xu2024large,   wei2024improving, xu2024code, li2024falcon, peng2024large, huang2024effi} \\ \cline{3-5} 
 &  & Memory   reduction & 1 & \cite{DBLP:journals/corr/abs-2407-14044} \\ \cline{3-5} 
 &  & Runtime   reduction (RTR) & 1 & \cite{DBLP:journals/corr/abs-2312-05657} \\ \hline
\multirow{2}{*}{Task-specific} & \multirow{2}{*}{10} & Percent optimized (\%OPT) & 9 & \cite{DBLP:journals/corr/abs-2309-14846,   gao2024searchbasedllmscodeoptimization, DBLP:journals/corr/abs-2109-13498,   DBLP:conf/nips/MadaanTGHGW0DPY23, DBLP:journals/corr/abs-2312-05657,   DBLP:conf/iclr/ShypulaMZ0GYHNR24, DBLP:journals/corr/abs-2406-11935, xu2024code,   zhang2024codedpo} \\ \cline{3-5} 
 &  & Area   Over the Convergence Curve (AOCC) & 1 & \cite{van2024llamea} \\ \hline
\multirow{2}{*}{Self-proposed} & \multirow{2}{*}{2} & Isomorphic Optimal Comparison   CodeBLEU (IOCCB) & 1 & \cite{pan2024measuringcodeefficiencyoptimization} \\ \cline{3-5} 
 &  & Normalized   Performance Index (NPI) & 1 & \cite{pan2024measuringcodeefficiencyoptimization}
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tb:evaluation_metric}
% \vspace{-0.3cm}
\end{table}

==> Tables/data_items.tex <==
\newcounter{itemcount}
\setcounter{itemcount}{1}
\begin{table}[t!]
  \centering
\small
\caption{The data items considered in this survey.}
  \begin{subtable}[t]{0.45\textwidth}
    \centering
\small
\begin{tabular}{lll}
\toprule
\multicolumn{1}{c}{\textbf{ID}} & \multicolumn{1}{c}{\textbf{Data Item}} & \multicolumn{1}{c}{\textbf{RQ}} \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Authors & N/A \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Title & N/A \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Publication venue & N/A \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Publication date & N/A \\ \hline
% $I_{\theitemcount\addtocounter{itemcount}{1}}$ & \# pages & N/A \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Base LM & RQ1 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & LM parameter size & RQ1 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & LM pretraining method & RQ1 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & LM fine-tuning method & RQ1 \\

\bottomrule
\end{tabular}
  \end{subtable}
  % \hspace{0.2cm}
  \begin{subtable}[t]{0.45\textwidth}
    \centering
\small
\begin{tabular}{lll}
\toprule
\multicolumn{1}{c}{\textbf{ID}} & \multicolumn{1}{c}{\textbf{Data Item}} & \multicolumn{1}{c}{\textbf{RQ}} \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & LM open accessibility & RQ1 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Code optimization method & RQ2 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Optimized language & RQ3 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Optimized performance & RQ3 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Downstream task & RQ3 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Existing dataset & RQ4 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Evaluation metric & RQ4 \\ \hline
$I_{\theitemcount\addtocounter{itemcount}{1}}$ & Real-world generalizability & RQ4 

\\ \bottomrule
\end{tabular}
  \end{subtable}
  \label{tb:data_items}
\end{table}

==> Tables/quality_assessment.tex <==
\newcounter{QACcount}
\setcounter{QACcount}{1}

\begin{table}[t!]
  \caption{Quality Assessment Criteria (QAC) and scoring metrics. The detailed scoring results can be found at: \textcolor{blue}{\url{https://github.com/gjz78910/CodeOpt-SLR}}}
% \vspace{-0.3cm}
\centering
\footnotesize
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lp{7cm}p{7cm}}
\toprule



\textbf{ID} & \textbf{Quality Assessment Criteria} & \textbf{Scoring Metric} \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & How many times has the paper been cited by other studies? & No=0, No more than 10 citations=1, More than 10 citations=2. \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & Does the paper provide a clear definition of the code optimization problem? & Not provided=0, Implicitly provided=1, Clearly provided=2. \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & Does the study provide a clear description of the proposed code optimization technique? & Not provided=0, Implicitly provided=1, Clearly provided=2. \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & Does the study compare the proposed model with other state-of-the-art baseline models? & No=0, Only one baseline=1, More than one baselines =2. \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & Are the experimental settings such as experimental environments, evaluation metrics, and dataset information described in detail? & Not described=0, Partially described=1, Fully described=2. \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & Are the key contributions and limitations of the study discussed? & Not discussed=0, Partially discussed=1, Fully discussed=2. \\ \hline
\emph{QAC$_{\theQACcount\addtocounter{QACcount}{1}}$} & Does the study provide resources to reproduce the experiment results? & No=0, Partially provided=1, Fully provided=2.
\\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tb:quality_assessment}
% \vspace{-0.3cm}
\end{table}

==> related_work.tex <==
\subsection{Related Works}
Before presenting LMs for code optimization, we first discuss prior studies on similar tasks that might be confused with code optimization, as well as a number of related surveys that investigate topics similar to this study. 

\subsubsection{LM related tasks}
LMs have been employed for a number of code-related tasks, including code generation, refactoring and repair, and performance modeling, described as follows. 

\textbf{LM-based code generation} translates a program specification into program code or executable binaries~\cite{coignion2024performance}. 
For example,~\citet{DBLP:journals/corr/abs-2203-07814} present AlphaCode, a novel LM-based system for code generation that achieves competitive performance based on natural language programming problems.~\citet{he2024cocost} design CoCoST to use LM in real-world programming scenarios by mimicking human coding processes, such as online searching and test case creation. Moreover,~\citet{liu2024evolution} introduce EoH, combining LMs and evolutionary computation methods for automatic algorithm design. 

\textbf{LM-based code refactoring}, similar to code editing \cite{DBLP:conf/sigsoft/GuptaKBCGKRS023}, code rewriting \cite{cummins2024don} or code transformation \cite{palkowski2024gpt}, focuses on restructuring the design, structure, and components of code, without explicitly addressing performance metrics~\cite{cordeiro2024empirical}. For instance,~\citet{li2023codeeditor} propose CodeEditor, which generates code mutations from real-world code and learns to edit them back to the original, thereby capturing effective refactoring patterns.~\citet{cummins2024don} emphasize generating refactoring transformations rather than directly rewriting code, allowing for easier inspection, debugging, and validation.

Additionally, efforts have been focused on \textbf{LM-based code repair}, where LMs are used to identify and fix defects, bugs, or errors in code to restore its intended functionality and ensure correctness~\cite{zhang2024systematic}. As examples,~\citet{DBLP:conf/sigsoft/JinSTSLSS23} employ a retrieval-based prompt augmentation technique and task-oriented fine-tuning in InferFix, leveraging bug-type annotations and extended source code context to enhance bug detection and repair processes, and~\citet{zhang2024autocoderover} leverage code representation through abstract syntax trees (ASTs) and employs spectrum-based fault localization to generate effective patches, resolving software issues efficiently.

Other works target \textbf{LM-based code performance modeling}, which involves analyzing and understanding the performance characteristics of code, serving as a potential component of code optimization~\cite{chen2024reasoning}. Among others,~\citet{DBLP:journals/corr/abs-2406-12806} introduce PerfSense, which leverages LM agents and prompt chaining techniques to analyze source code and classify configurations as performance-sensitive or insensitive, thereby enhancing performance analysis.
Besides, in the work by~\citet{DBLP:journals/corr/abs-2306-17281}, an LM is fine-tuned on a curated dataset containing HPC and scientific codes, and is employed to predict the relative performance impact of changes made to the source code. 

While the above studies are related to code optimization to some extent, they are not included in this survey because their primary focuses are different from our definition of code optimization\footnote{Note that although some studies do not explicitly define their task as code optimization, we have included them in this survey if in any steps the performance of existing code is improved, typical examples will be some studies for code editing, code refinement, and some code generation studies with iterative performance improvements.}. This survey aims to address this gap by focusing exclusively on the application of LMs for optimizing the performance of existing code or programs.

\subsubsection{Related surveys}
To the best of our knowledge, the most relevant surveys to ours are those focusing on \textbf{LMs for evolutionary algorithms (EAs)}, which involve solving optimization problems by iteratively improving a population of candidates through mechanisms inspired by biological evolution, such as selection, mutation, and crossover. Specifically,~\citet{huang2024large} discuss the role of LMs in solving complex optimization problems through evolutionary mechanisms and provide future directions in this application, and~\citet{wu2024evolutionary} explore the collaborative strengths of LMs and EAs in three aspects: LM-enhanced EA, EA-enhanced LM, and their applications in optimization tasks. However, these surveys only cover a broad range of optimization problems, not specializing in enhancing the performance of existing programs.

Besides, previous surveys have typically focused on \textbf{code optimization using traditional methods} involving compilers, ML, and DL techniques~\cite{li2020deep, wang2018machine, bhatsurvey, wan2024deep, sun2024survey}. For instance,~\citet{wang2018machine} discuss the integration of ML into compiler optimization, highlighting its evolution over the past 50 years and its current status as a mainstream research area. More recently,~\citet{wan2024deep} conduct a comprehensive survey on deep learning for code intelligence, covering aspects such as code representations, DL techniques, application tasks, and public datasets.
% ashouri2018survey, allamanis2018survey, ghaemi2024transformers

Moreover, a few surveys have investigated the utilization of \textbf{LMs for code-related tasks}, including general code intelligence~\cite{DBLP:journals/corr/abs-2311-10372, DBLP:journals/entropy/WongGHHT23}, code generation~\cite{DBLP:journals/corr/abs-2406-00515, chen2024survey}, and code repair~\cite{zhang2024systematic}. In particular,~\citet{zhang2023unifying} review the evolution of LM-based techniques for code processing tasks from pre-trained Transformer to advanced retrieval and agentic approaches, and~\citet{chen2024survey} survey current methods and metrics for assessing code generation capabilities, identifying their limitations and proposing directions for future improvements.
% zhang2023unifying, joel2024survey, DBLP:journals/corr/abs-2407-07064

Additionally, there are several surveys on the use of \textbf{LMs in general software engineering tasks}. For example,~\citet{hou2024largelanguagemodelssoftware} provide a comprehensive understanding of how LMs can optimize SE processes and outcomes, addressing gaps in existing research. Similarly,~\citet{DBLP:conf/fose-ws/FanGHLSYZ23} provide a comprehensive overview of the current state of research and future directions in LM-based software engineering, and~\citet{DBLP:journals/corr/abs-2404-04566} propose a vision for the future of LLM4SE that includes a roadmap for research directions aimed at improving efficiency and reducing carbon emissions associated with LMs.

% introduce why there is a knowledge gap for a survey specifically focus on LMs for code optimization
Despite the existence of comprehensive surveys, there is a notable knowledge gap when it comes to a focused survey on the use of LMs specifically for code optimization. Therefore, this survey addresses this gap by systematically reviewing the current state of research and applications of LMs in code optimization, identifying the strengths and limitations of existing approaches, and providing guidance for future research directions.


% ~\citet{huang2024generative} present a literature review on generative software engineering, focusing on a comprehensive analysis of the development process from pre-trained models to LLMs,

% Furthermore, many studies are surveying \textbf{the most recent LMs}~\cite{hadi2024large, zhao2023survey, patil2024review, hadi2023survey, minaee2024large}.

% Moreover, there are also surveys on \textbf{LMs for various domains}, such as cyber security~\cite{DBLP:journals/corr/abs-2312-02003, DBLP:journals/corr/abs-2405-04760}, HPC~\cite{DBLP:journals/corr/abs-2402-02018}, education~\cite{rahman2023chatgpt}, and NLP~\cite{DBLP:journals/csur/MinRSVNSAHR24}.

% Besides, several survey studies exist for \textbf{specific LM-related techniques}, like LLM agents~\cite{liu2024large}, LLM serving~\cite{DBLP:journals/corr/abs-2312-15234}, and LLM prompting~\cite{li2024towards}.






==> standalone.tex <==
% \documentclass[a4paper,10pt]{article}
% \usepackage{amsmath,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{booktabs}
% \usepackage{tikz,pgfplots}
% \usepackage{standalone}
% \usepackage[most]{tcolorbox}
% \usepackage{csquotes}
% \usepackage{url}
% \usepackage{multirow}
% \usetikzlibrary{arrows.meta}
% \usepackage{fancyhdr}
% \usepackage{threeparttable}
% \usepackage{subcaption}
% \usepackage{makecell}
% \usepackage{hyperref}
% \usepackage{newtxmath}
% \usepackage{pgf-pie}
% \usepackage{multirow}
% \usepackage{pifont} % Provides check marks and crosses
% \usepackage{xspace}

% \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% \newcommand{\keybox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% \em #1
% \end{tcolorbox}
% }

% \begin{document}






% \begin{table}[t!]
%   \caption{The datasets and benchmarks for code optimization (one study might be in multiple categories).}
% % \vspace{-0.3cm}
% \centering
% \footnotesize
% \begin{adjustbox}{width=\linewidth,center}
% \begin{tabular}{lllllllll}
% \toprule
% \textbf{Category} & \textbf{Total \#} & \textbf{Dataset} & \textbf{Source} & \textbf{Size} & \textbf{Languages} & \textbf{Performance} & \textbf{Repo} & \textbf{Reference} \\ \hline
% \multirow{16}{1.6cm}{Competitive programming tasks} & \multirow{16}{*}{31} & HumanEval~\cite{DBLP:journals/corr/abs-2107-03374} & Hand-crafted by experts & 164 programming tasks & Python & Correctness & \href{https://github.com/openai/human-eval}{Link} & \cite{DBLP:journals/corr/abs-2405-15189,   DBLP:conf/nips/ShinnCGNY23, DBLP:journals/corr/abs-2406-12502, li2024falcon,   huang2024effi, zhang2024codedpo} \\ \cline{3-9} 
%  &  & MBPP~\cite{DBLP:journals/corr/abs-2108-07732} & Programming problems & 974 programming tasks & Python & Correctness & \href{https://github.com/google-research/google-research/tree/master/mbpp}{Link} & \cite{DBLP:journals/corr/abs-2405-15189,   DBLP:conf/nips/ShinnCGNY23, DBLP:journals/corr/abs-2406-12502, li2024falcon,   zhang2024codedpo} \\ \cline{3-9} 
%  &  & PIE~\cite{DBLP:conf/iclr/ShypulaMZ0GYHNR24} & CodeNet & 77K pairs of slow-fast code & C++ & Runtime & \href{https://github.com/LearningOpt/pie?tab=readme-ov-file#dataset}{Link} & \cite{gao2024searchbasedllmscodeoptimization,   DBLP:conf/nips/MadaanTGHGW0DPY23, DBLP:journals/corr/abs-2312-05657,   DBLP:conf/iclr/ShypulaMZ0GYHNR24} \\ \cline{3-9} 
%  &  & EffiBench~\cite{DBLP:journals/corr/abs-2402-02037} & Leetcode & 1K efficiency-critical coding   problems & Python & Runtime, memory & \href{https://huggingface.co/datasets/DONG19/EffiBench}{Link} & \cite{DBLP:journals/corr/abs-2405-15189,   huang2024effi} \\ \cline{3-9} 
%  &  & CodeContests~\cite{DBLP:journals/corr/abs-2203-07814} & Aizu Online Judge, AtCoder & 13,610 samples & Python, C++, Java & Runtime, memory & \href{https://github.com/google-deepmind/code_contests}{Link} & \cite{DBLP:conf/apsec/ShirafujiOSMW23,   DBLP:journals/corr/abs-2401-08500} \\ \cline{3-9} 
%  &  & LeetcodeHardGym~\cite{DBLP:conf/nips/ShinnCGNY23} & Leetcode & 40 questions & Python, Rust & Runtime & \href{https://github.com/GammaTauAI/leetcode-hard-gym}{Link} & \cite{DBLP:conf/nips/ShinnCGNY23,   DBLP:journals/corr/abs-2406-07496} \\ \cline{3-9} 
%  &  & ECCO~\cite{DBLP:journals/corr/abs-2407-14044} & CodeNet & 50K solution pairs & Python & Runtime, memory & \href{https://github.com/CodeEff/ECCO}{Link} & \cite{DBLP:journals/corr/abs-2407-14044} \\ \cline{3-9} 
%  &  & FunSearch~\cite{DBLP:journals/nature/RomeraParedesBNBKDREWFKF24} & Algorithmic problems & $10^6$ samples & Python & Complexity, readability,   maintainability & \href{https://github.com/google-deepmind/funsearch}{Link} & \cite{DBLP:journals/nature/RomeraParedesBNBKDREWFKF24} \\ \cline{3-9} 
%  &  & Supersonic~\cite{DBLP:journals/corr/abs-2309-14846} & CodeNet & 314,435 samples & C, C++ & Runtime, memory & \href{https://github.com/ASSERT-KTH/Supersonic}{Link} & \cite{DBLP:journals/corr/abs-2309-14846} \\ \cline{3-9} 
%  &  & GEC~\cite{DBLP:conf/internetware/PanL23} & CodeForces & 31,577 pairs of slow-fast   code & Python & Runtime & \href{https://github.com/CodeGeneration2/GEC-Dataset}{Link} & \cite{pan2024ecodemasteringefficientcode} \\ \cline{3-9} 
%  &  & CodeNet~\cite{DBLP:journals/corr/abs-2105-12655} & AIZU Online Judge, AtCoder & 14 million samples & C++, C, C\#, Python, Java... & Runtime, memory, code size & \href{https://developer.ibm.com/exchanges/data/all/project-codenet/}{Link} & \cite{DBLP:conf/hpec/GuoM22} \\ \cline{3-9} 
%  &  & ACEOB~\cite{pan2024measuringcodeefficiencyoptimization} & CodeForces & 95,359 pairs of   efficient-inefficient code & Python & Runtime & \xmark & \cite{pan2024measuringcodeefficiencyoptimization} \\ \cline{3-9} 
%  &  & APPS~\cite{hendrycks2021measuring} & Coding websites & 10k coding problems & Python & Correctness & \href{https://github.com/hendrycks/apps?form=MG0AV3}{Link} & \cite{li2024falcon} \\ \cline{3-9} 
%  &  & Effi-Code~\cite{huang2024effi} & Coding datasets & 9,451 tasks & Python & Runtime, memory & \href{https://github.com/huangd1999/Effi-Code}{Link} & \cite{huang2024effi} \\ \cline{3-9} 
%  &  & SAPIE~\cite{xu2024code} & CodeNet & 77k pairs of slow-fast code & C++ & Runtime & \xmark & \cite{xu2024code} \\ \cline{3-9} 
%  &  & PIE-problem~\cite{DBLP:journals/corr/abs-2406-11935} & CodeNet & 18,242 pairs of slow-fast   code & C++ & Runtime & \xmark & \cite{DBLP:journals/corr/abs-2406-11935} \\ \hline
% \multirow{13}{1.6cm}{Real-world programs} & \multirow{13}{*}{17} & PolyBench~\cite{DBLP:conf/cc/Abella-Gonzalez21} & Various application domains & 30 numerical polyhedral kernels & Python, C & Runtime, memory & \href{https://github.com/UDC-GAC/polybench-python}{Link} & \cite{DBLP:journals/corr/abs-2408-03408,   DBLP:journals/corr/abs-2404-18864, DBLP:journals/pacmpl/YeZSS23} \\ \cline{3-9} 
%  &  & DeepDev-PERF~\cite{DBLP:conf/sigsoft/GargMCSW22} & GitHub & 50 open-source repositories & C\# & CPU, memory & \xmark & \cite{DBLP:journals/corr/abs-2306-17077,   DBLP:conf/sigsoft/GargMCSW22} \\ \cline{3-9} 
%  &  & LLM4Compiler~\cite{DBLP:journals/corr/abs-2309-07062} & GitHub, synthesis & 1 million  functions & LLVM-IR & Code size & \xmark & \cite{DBLP:journals/corr/abs-2309-07062,   DBLP:journals/corr/abs-2403-14714} \\ \cline{3-9} 
%  &  & AnghaBench~\cite{DBLP:conf/cgo/SilvaKMRGP21} & GitHub & 1 million samples & C & Runtime, code size & \href{http://cuda.dcc.ufmg.br/angha/benchmarks}{Link} & \cite{DBLP:conf/hpec/GuoM22} \\ \cline{3-9} 
%  &  & InstructCoder~\cite{li2024instructcoderinstructiontuninglarge} & GitHub & 114K instruction-input-output   triplets & Python & Complexity, readability,   maintainability & \href{https://github.com/qishenghu/InstructCoder}{Link} & \cite{li2024instructcoderinstructiontuninglarge} \\ \cline{3-9} 
%  &  & BetterPython~\cite{shivashankar2024betterpythonprogrammingall} & CommitPackFT, CodeAlpaca & 34,139 samples & Python & Complexity, readability,   maintainability & \href{https://zenodo.org/records/10940620}{Link} & \cite{shivashankar2024betterpythonprogrammingall} \\ \cline{3-9} 
%  &  & RewriterBench~\cite{yao2024rtlrewritermethodologieslargemodels} & Industry cases & 55 cases & RTL & Synthesis performance & \href{https://github.com/yaoxufeng/RTLRewriter-Bench}{Link} & \cite{yao2024rtlrewritermethodologieslargemodels} \\ \cline{3-9} 
%  &  & ST to   C~\cite{DBLP:journals/concurrency/HanLDLZ24} & Industry cases & 3 case studies & Structured Text (ST), C & Readability, maintainability & \xmark & \cite{DBLP:journals/concurrency/HanLDLZ24} \\ \cline{3-9} 
%  &  & PandasEval~\cite{jain2022jigsaw} & StackOverflow & 89 Pandas tasks & Python & Correctness & \href{https://github.com/microsoft/JigsawDataset}{Link} & \cite{jain2022jigsaw} \\ \cline{3-9} 
%  &  & Big   Assembly~\cite{DBLP:journals/corr/abs-2109-13498} & GitHub & 25,141 assembly functions & x86-64 assembly language & CPU-clock cycles & \xmark & \cite{DBLP:journals/corr/abs-2109-13498} \\ \cline{3-9} 
%  &  & Big-DS-1000~\cite{qu2024dynamic} & StackOverflow & 1000 data science problems & Python & Runtime & \xmark & \cite{qu2024dynamic} \\ \cline{3-9} 
%  &  & DS-1000~\cite{lai2023ds} & StackOverflow & 1000 data science problems & Python & Correctness & \href{https://ds1000-code-gen.github.io/}{Link} & \cite{zhang2024codedpo} \\ \cline{3-9} 
%  &  & Priority   Sampling~\cite{DBLP:conf/euromlsys/GrubisicSSLMC24} & GitHub & 50K functions & LLVM-IR & Code size & \xmark & \cite{DBLP:conf/euromlsys/GrubisicSSLMC24} \\ \hline
% \multirow{2}{1.6cm}{Synthetic programs} & \multirow{2}{*}{2} & TSVC~\cite{maleki2011evaluation} & Synthesis & 149 test cases & C & Runtime, code size & \href{https://github.com/UoB-HPC/TSVC_2}{Link} & \cite{DBLP:journals/corr/abs-2406-04693} \\ \cline{3-9} 
%  &  & CSmith~\cite{DBLP:conf/pldi/YangCER11} & Synthesis & Unlimited & C & Runtime & \href{https://github.com/csmith-project/csmith}{Link} & \cite{DBLP:conf/hpec/GuoM22}
% \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{tb:datasets}
% % \vspace{-0.3cm}
% \end{table}





% \begin{figure}[!t]
% \centering
% \includestandalone[width=0.5\columnwidth]{Figures/RQ_real_world}
% \vspace{-0.3cm}
%   \caption{Distribution of evaluation on real-world programs.}
%  \label{fig:real_world}
%  \end{figure}















% % \bibliographystyle{plain}
% % \bibliography{references}
% \end{document}

==> standalone_methodology.tex <==
% \documentclass[a4paper,10pt]{article}
% %\usepackage{pxfonts}
% \textwidth=148mm
% \textheight=250mm
% \voffset -25mm
% \hoffset -10mm
% \renewcommand{\baselinestretch}{1.1}
% \setlength{\parskip}{0.5\baselineskip}
% % \setlength\parindent{0pt}

% \usepackage{amsmath,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{booktabs}
% \usepackage{tikz,pgfplots}
% \usepackage{standalone}
% \usepackage[most]{tcolorbox}
% \usepackage{csquotes}
% \usepackage{url}
% \usepackage{multirow}
% \usetikzlibrary{arrows.meta}
% \usepackage{fancyhdr}
% \usepackage{threeparttable}
% \usepackage{subcaption}
% \usepackage{makecell}
% \usepackage{hyperref}
% \usepackage{newtxmath}
% \usepackage{pgf-pie}
% \usepackage{multirow}
% \usepackage{fontawesome5}
% \usepackage{pifont} % Provides check marks and crosses
% \usepackage{xspace}
% \usepackage{natbib}

% \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% % \newcommand{\keybox}[1]{
% % \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% % \em #1
% % \end{tcolorbox}
% % }

% \lstset{
%     language=Python,
%     basicstyle=\ttfamily\footnotesize,
%     keywordstyle=\color{blue},
%     stringstyle=\color{red},
%     commentstyle=\color{green},
%     morecomment=[l][\color{magenta}]{\#},
%     numbers=left,
%     numberstyle=\tiny\color{gray},
%     stepnumber=1,
%     numbersep=5pt,
%     showstringspaces=false,
%     breaklines=true,
%     frame=single,
%     backgroundcolor=\color{white},
%     captionpos=b
% }


% \makeatletter
% \tcbset{
%     myhbox/.style 2 args={%
%         enhanced, 
%         breakable,
%         colback=white,
%         colframe=cerublue!70,
%         attach boxed title to top left={yshift*=-\tcboxedtitleheight}, 
%         title={#2},
%         boxed title size=title,
%         boxed title style={%
%             sharp corners, 
%             rounded corners=northwest, 
%             colback=tcbcolframe, 
%             boxrule=0pt,
%         },
%         underlay boxed title={%
%             \path[fill=tcbcolframe] (title.south west)--(title.south east) 
%                 to[out=0, in=180] ([xshift=5mm]title.east)--
%                 (title.center-|frame.east)
%                 [rounded corners=\kvtcb@arc] |- 
%                 (frame.north) -| cycle; 
%         },
%         #1
%     }
% }   
% \makeatother

% \newtcolorbox{myhbox}[2][]{%
%     myhbox={#1}{#2}
% }

% \newcounter{findingcount}
% \setcounter{findingcount}{1} 
% \newcounter{suggestioncount}
% \setcounter{suggestioncount}{1}

% \newcommand{\keybox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=beaublue]
% \em #1
% \end{tcolorbox}
% }

% \newcommand{\suggestbox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=dollarbill!50]
% \em #1
% \end{tcolorbox}
% }
% % \usepackage{amsmath,amsfonts}
% % \usepackage{algorithmic}
% % \usepackage{graphicx}
% % \usepackage{textcomp}
% % \usepackage{xcolor}
% % \usepackage{booktabs}
% % \usepackage{tikz,pgfplots}
% % \usepackage{standalone}
% % \usepackage[most]{tcolorbox}
% % \usepackage{csquotes}
% % \usepackage{url}
% % \usepackage{multirow}
% % \usetikzlibrary{arrows.meta}
% % \usepackage{fancyhdr}
% % \usepackage{threeparttable}
% % \usepackage{subcaption}
% % \usepackage{makecell}
% % \usepackage{hyperref}
% % \usepackage{newtxmath}
% % \usepackage{pgf-pie}
% % \usepackage{multirow}
% % \usepackage{pifont} % Provides check marks and crosses
% % \usepackage{xspace}
% % \usepackage{natbib}

% % \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% % \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% % \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% % \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% % \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% % \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% % \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% % \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% % \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% % \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% % \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% % \newcommand{\keybox}[1]{
% % \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% % \em #1
% % \end{tcolorbox}
% % }



% \begin{document}





% \begin{figure}[!t]
% \centering
% \includegraphics[width=\columnwidth]{Figures/methodology}
% % ~\vspace{-0.2cm}
%     \caption{Overview of the survey methodology used in this study.}
%  \label{fig:methodology}
%  \end{figure}

% \appendix
% \section{Methodology}
% We now describe the methodology used to collect literature and data and perform the analysis. Specifically, we follow the widely recognized guidelines for SLRs in Software Engineering proposed by Kitchenham and Charters~\cite{keele2007guidelines}, which have also been adopted by numerous SLRs~\cite{DBLP:journals/corr/Gong24Deep, hou2024largelanguagemodelssoftware, DBLP:journals/tse/WangHGGZFSLZN23, zhang2024systematic, DBLP:journals/corr/abs-2405-04760}. The methodology comprises three key stages, as illustrated in Figure~\ref{fig:methodology}.
% Note that throughout all stages, we follow the iterative procedures among co-authors of the article:
% \begin{enumerate}
%     \item The first author performs initial actions and shares the results with one of the co-authors;
%     \item The co-author assists the first author with all needed actions and reviews the results;
%     \item If the two authors make an agreement, the results of all actions are presented and reviewed by all the rest of the co-authors; otherwise, go to (1);
%     \item If agreements are achieved, go to the next stage, other wise, restart from (1).
% \end{enumerate}
% In the following sub-sections, we will introduce each stage in detail.

% \subsection{Search Strategy}
% \subsubsection{Search string}

% To ensure a comprehensive and accurate search, we began by defining a search string using the ``quasi-gold standard'' (QGS)~\cite{DBLP:journals/infsof/ZhangBT11}, an approach commonly used in modern surveys~\cite{hou2024largelanguagemodelssoftware, DBLP:journals/tse/WangHGGZFSLZN23, zhang2024systematic, DBLP:journals/corr/abs-2405-04760, DBLP:journals/corr/Gong24Deep}. In particular, we first manually collected 10 high-quality studies\footnote{Marked in \url{https://github.com/gjz78910/CodeOpt-SLR/blob/main/Quality_assessment_results.xlsx}.} based on their impact, citation count, and relevance to the topic of code optimization using LMs. From these QGS studies, we extracted keywords and phrases central to our research objectives and created the first draft search string. Then, we iteratively performed searches using Google Scholar and refined the search string until the sensitivity (\%) $s$ of the search is higher than 80\%~\cite{DBLP:journals/infsof/ZhangBT11}, which is computed using the equation as follows:

% % Then, we iteratively performed searches using Google Scholar and refined the search string until the sensitivity of the search~\cite{DBLP:journals/infsof/ZhangBT11} is over 80\%.

% \begin{equation}
% s = \frac{\text{\# relevant studies searched}}{\text{Total \# relevant studies in the QGS}} \times 100
% \end{equation}

% Formally, the search string produced by the QGS methodology is: 
% \begin{tcbitemize}[%
%     raster columns=1, 
%     raster rows=1
%     ]
%   \tcbitem[myhbox={}{Search String}]   \textit{``language models'' AND (``code optimization'' OR ``compiler optimization''OR ``optimize code'' OR ``optimizing code'' OR ``code performance optimization'') }
% \end{tcbitemize}

% \subsubsection{Automatic search}

% Using the defined search string, we conducted automatic searches on seven popular academic indexing engines~\cite{hou2024largelanguagemodelssoftware, DBLP:journals/tse/WangHGGZFSLZN23, zhang2024systematic, DBLP:journals/corr/abs-2405-04760, DBLP:journals/corr/abs-2401-14617}, as shown in Figure~\ref{fig:methodology}, i.e., Google Scholar, IEEE Xplore, ACM Digital Library, Science Direct, Springer, and WILEY.

% To ensure maximum coverage, we included both American and British spellings for keywords like ``optimizing'' and ``optimising'', and replaced ``code'' with ``program'' and ``software''. Since the field of language models is developing quickly, we regularly updated the search results until November 2024 to ensure the most recent advancements were captured. This process resulted in 2,310 searched studies in total. 

% \subsubsection{Snowballing search}

% Following the automatic search, we conducted a manual snowballing search based on the 10 QGS studies using Google Scholar and Connected Papers, involving both forward snowballing (identifying papers that cite the QGS) and backward snowballing (reviewing the references cited by the QGS). This is effective to uncover studies that are relevant but might not be captured through keyword searches~\cite{hou2024largelanguagemodelssoftware, zhang2024systematic, DBLP:journals/corr/abs-2405-04760, DBLP:journals/corr/abs-2401-14617, DBLP:journals/tosem/WatsonCNMP22}, such as code generation studies that optimize code performance as part of their iterative workflow~\cite{peng2024large, han2024generating}. In summary, the snowballing process led to 36 extra searched studies.

% % Our approach was guided by techniques outlined in “A Systematic Literature Review on the Use of Deep Learning in Software Engineering Research”. This iterative process helped ensure that we did not miss any significant contributions to the field.

% % Refer to 'A Systematic Literature Review on the Use of Deep Learning in Software Engineering Research'

% \subsection{Study Selection}
% % In the next stage, I performed study selection using a list of inclusion and exclusion criteria.
% \subsubsection{Inclusion and exclusion criteria}
% In the second stage, we filtered duplicate and irrelevant searched studies, and performed rigorous study selection using a list of inclusion and exclusion criteria, following the SLR guideline and previous SLR studies~\cite{keele2007guidelines}. By adhering to these criteria, we aim to identify a specialized and reliable subset of the current state of research and practice in this area, serving as the primary studies to be reviewed. In particular, the inclusion criteria include:
% \begin{itemize} 
%     \item[\cmark] The paper presents a novel code optimization method. 
%     \item[\cmark] The proposed method uses language models. 
%     \item[\cmark] The paper aims to optimize at least one of the non-functional performance metrics of the original code. 
%     \item[\cmark] The paper conducts rigorous experiments to evaluate the proposed method. 
% \end{itemize}

% Nevertheless, this still led to irrelevant studies to our research topic, therefore, we performed further filtering using the following exclusion criteria:
% \begin{itemize} 
%     \item[\xmark] The paper does not use code as input in any part of the pipeline. 
%     \item[\xmark] The paper is focused on improving functionalities of code, or fixing code bugs. 
%     \item[\xmark] The paper is a poster or abstract, without technical details and experimental results. 
%     \item[\xmark] The paper is not written in English. 
% \end{itemize}

% \subsubsection{Quality assessment}
% Moreover, since many of the primary studies are not peer-reviewed, we conducted a comprehensive quality assessment to examine their quality and to ensure the quality of our survey and the reliability of the findings. Specifically, we removed studies with scores equal to or less than one, and Table~\ref{tb:quality_assessment} presents the Quality Assessment Criteria (QAC) we used. As a result, 53 primary studies were selected for the next stage of detailed review and data collection.

% \input{Tables/quality_assessment}

% % \begin{figure}[!t]
% % \centering
% % \includestandalone[width=0.95\columnwidth]{Figures/quality_assessment_scores}
% % ~\vspace{-0.2cm}
% %     \caption{Average scores for each quality assessment question.}
% %  \label{fig:avg_score}
% %  \end{figure}



% % Refer to ’Topology-aware Federated Learning in Edge Computing: A Comprehensive Survey’

% % 'Predictive Models in Software Engineering: Challenges and Opportunities'

% \subsection{Research Questions and Data Collection}

% In the third stage, to guide our systematic literature review, we formulated a set of four primary research questions aimed at addressing the key aspects of using LMs for code optimization, to answer this, we identified a few key sub-questions, carefully reviewed the primary studies and collected data items accordingly.

% \keybox{
% \textbf{RQ1:} What were the characteristics of the LMs used for code optimization?
% }

% The first RQ aims to explore the foundational attributes of the LMs employed for code optimization, which includes collecting data about the base models, their sizes, whether they are open source, and how they were pre-trained and fine-tuned.

% \keybox{
% \textbf{RQ2:} How were LMs applied to code optimization tasks?
% }

% This question seeks to identify and categorize the practical roles and applications of LMs in the code optimization pipeline. It involved gathering insights into common challenges addressed by LMs, the specific optimization techniques employed, and the role of LMs within the optimization workflow.


% \keybox{
% \textbf{RQ3:} What programming languages and performance metrics were considered in LM-based code optimization?
% }

% The aim of this question is to provide a comprehensive view of the code optimization problem. To address this, we collected data on the programming languages and performance metrics involved in the primary studies.

% \keybox{
% \textbf{RQ4:} How were the proposed code optimization methods evaluated?
% }

% This final question focuses on understanding the evaluation methodologies used to validate LM-driven code optimization techniques. It involved analyzing the datasets utilized, the application of optimization methods to real-world programs, and the evaluation metrics.


% % To answer the above RQs, we carefully read each primary study and collected a set of data items, as shown in Table~\ref{tb:data_items}.


% % \input{Tables/data_items}

% % For RQ1, we collected information on the base models used, their sizes, whether they are open source, and details on their pre-training and fine-tuning processes.

% % For RQ2, we gathered data on the specific techniques employed for code optimization, the datasets utilized, the design of the models, and the formulation of the optimization problems. This included identifying the various methodologies and frameworks applied in the studies, as well as any unique approaches or innovations introduced.

% % For RQ3, we documented the programming languages targeted by the LMs, the performance metrics used to evaluate the optimization, and the specific application fields or downstream tasks. This involved noting the diversity of languages and metrics, as well as the relevance of the optimization tasks to real-world applications.

% % For RQ4, we extracted information on the evaluation methods used in the studies, the datasets employed for benchmarking, and the overall evaluation pipelines. This included details on the experimental setups, the criteria for success, and any standardized benchmarks or datasets referenced in the literature.

% % \begin{figure}[!t]
% % \centering
% % \includestandalone[width=0.6\columnwidth]{Figures/distribution_venue}
% % % \vspace{-0.7cm}
% %   \caption{Distribution of publication venues.}
% %  \label{fig:distribution_venue}
% %  \end{figure}

% \begin{figure}[!t]
% \centering
% \begin{minipage}{0.5\textwidth}
% \includestandalone[width=\columnwidth]{Figures/distribution_venue}
% \vspace{-0.7cm}
%   \caption{Distribution of publication venues.}
%  \label{fig:distribution_venue}
%   \end{minipage}
% ~\hspace{0.5cm}
% \begin{minipage}{0.4\textwidth}
% \vspace{0.8cm}
% \includestandalone[width=\columnwidth]{Figures/distribution_year}
% \vspace{0cm}
%   \caption{Distribution of primary studies over years (till November 2024).}
%  \label{fig:distribution_year}
%   \end{minipage}
%  \end{figure}

% \subsection{Statistics of Primary Studies}
 
% Figure~\ref{fig:distribution_venue} provides a detailed view of the distribution of the reviewed primary studies across various publication venues. Notably, the largest portion of studies (24 or 45\%) were sourced from arXiv as preprints, suggesting ongoing and rapidly developing work in this area. Three other significant venues include NeurIPS~\cite{DBLP:journals/corr/abs-2405-15189, DBLP:conf/nips/MadaanTGHGW0DPY23, DBLP:conf/nips/ShinnCGNY23}, ICSE~\cite{jain2022jigsaw, gao2024searchbasedllmscodeoptimization}, and ICLR~\cite{DBLP:conf/iclr/ShypulaMZ0GYHNR24, ishida2024langpropcodeoptimizationframework}, reflecting the relevance of machine learning and software engineering in the context of code optimization. The remaining studies are spread across 22 conferences and journals (one study each), such as Nature~\cite{DBLP:journals/nature/RomeraParedesBNBKDREWFKF24}, TSE~\cite{DBLP:journals/corr/abs-2309-14846}, PACMPL~\cite{DBLP:journals/pacmpl/YeZSS23}, and HPEC~\cite{DBLP:conf/hpec/GuoM22}, and four workshops like LAD~\cite{xu2024optimizing, DBLP:journals/corr/abs-2408-03408, pan2024measuringcodeefficiencyoptimization}. This diversity highlights that the topic is addressed not only in AI and SE-specific forums but also in broader scientific and engineering communities.

% Moreover, Figure~\ref{fig:distribution_year} presents the distribution of studies by year, where the majority of studies, 79\%, were published in 2024, totaling 42 studies. In comparison, 2023 contributed 13\% (seven studies), and 2022 accounted for only 8\% (four studies). This significant increase suggests a surge in interest in LM-based code optimization research recently.


% % \begin{figure}[!t]
% % \centering
% % \includestandalone[width=0.5\columnwidth]{Figures/distribution_year}
% %   \caption{Distribution of primary studies over years (till November 2024).}
% %  \label{fig:distribution_year}
% %  \end{figure}

% % \subsection{The Taxonomy Overview}
% % In Figure~\ref{fig:overview}, we give an overview of the taxonomy for all RQs. Subsequently, we will delineate the survey results and discussions of each RQ separately in the following sections.


% % \begin{figure}[!t]
% % \centering
% % \includegraphics[width=0.8\columnwidth]{Figures/taxonomy.pdf}
% % % ~\vspace{-0.2cm}
% %     \caption{Overview of the taxonomy for the RQs (one study might be in multiple categories).}
% %  \label{fig:overview}
% %  \end{figure}




% \bibliographystyle{plain}
% \bibliography{references}
% \end{document}

==> standalone_related_work.tex <==
% \documentclass[a4paper,10pt]{article}
% %\usepackage{pxfonts}
% \textwidth=148mm
% \textheight=250mm
% \voffset -25mm
% \hoffset -10mm
% \renewcommand{\baselinestretch}{1.1}
% \setlength{\parskip}{0.5\baselineskip}
% % \setlength\parindent{0pt}

% \usepackage{amsmath,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{booktabs}
% \usepackage{tikz,pgfplots}
% \usepackage{standalone}
% \usepackage[most]{tcolorbox}
% \usepackage{csquotes}
% \usepackage{url}
% \usepackage{multirow}
% \usetikzlibrary{arrows.meta}
% \usepackage{fancyhdr}
% \usepackage{threeparttable}
% \usepackage{subcaption}
% \usepackage{makecell}
% \usepackage{hyperref}
% \usepackage{newtxmath}
% \usepackage{pgf-pie}
% \usepackage{multirow}
% \usepackage{fontawesome5}
% \usepackage{pifont} % Provides check marks and crosses
% \usepackage{xspace}
% \usepackage{natbib}

% \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% % \newcommand{\keybox}[1]{
% % \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% % \em #1
% % \end{tcolorbox}
% % }

% \lstset{
%     language=Python,
%     basicstyle=\ttfamily\footnotesize,
%     keywordstyle=\color{blue},
%     stringstyle=\color{red},
%     commentstyle=\color{green},
%     morecomment=[l][\color{magenta}]{\#},
%     numbers=left,
%     numberstyle=\tiny\color{gray},
%     stepnumber=1,
%     numbersep=5pt,
%     showstringspaces=false,
%     breaklines=true,
%     frame=single,
%     backgroundcolor=\color{white},
%     captionpos=b
% }


% \makeatletter
% \tcbset{
%     myhbox/.style 2 args={%
%         enhanced, 
%         breakable,
%         colback=white,
%         colframe=cerublue!70,
%         attach boxed title to top left={yshift*=-\tcboxedtitleheight}, 
%         title={#2},
%         boxed title size=title,
%         boxed title style={%
%             sharp corners, 
%             rounded corners=northwest, 
%             colback=tcbcolframe, 
%             boxrule=0pt,
%         },
%         underlay boxed title={%
%             \path[fill=tcbcolframe] (title.south west)--(title.south east) 
%                 to[out=0, in=180] ([xshift=5mm]title.east)--
%                 (title.center-|frame.east)
%                 [rounded corners=\kvtcb@arc] |- 
%                 (frame.north) -| cycle; 
%         },
%         #1
%     }
% }   
% \makeatother

% \newtcolorbox{myhbox}[2][]{%
%     myhbox={#1}{#2}
% }

% \newcounter{findingcount}
% \setcounter{findingcount}{1} 
% \newcounter{suggestioncount}
% \setcounter{suggestioncount}{1}

% \newcommand{\keybox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=beaublue]
% \em #1
% \end{tcolorbox}
% }

% \newcommand{\suggestbox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=dollarbill!50]
% \em #1
% \end{tcolorbox}
% }
% % \usepackage{amsmath,amsfonts}
% % \usepackage{algorithmic}
% % \usepackage{graphicx}
% % \usepackage{textcomp}
% % \usepackage{xcolor}
% % \usepackage{booktabs}
% % \usepackage{tikz,pgfplots}
% % \usepackage{standalone}
% % \usepackage[most]{tcolorbox}
% % \usepackage{csquotes}
% % \usepackage{url}
% % \usepackage{multirow}
% % \usetikzlibrary{arrows.meta}
% % \usepackage{fancyhdr}
% % \usepackage{threeparttable}
% % \usepackage{subcaption}
% % \usepackage{makecell}
% % \usepackage{hyperref}
% % \usepackage{newtxmath}
% % \usepackage{pgf-pie}
% % \usepackage{multirow}
% % \usepackage{pifont} % Provides check marks and crosses
% % \usepackage{xspace}
% % \usepackage{natbib}

% % \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% % \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% % \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% % \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% % \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% % \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% % \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% % \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% % \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% % \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% % \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% % \newcommand{\keybox}[1]{
% % \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% % \em #1
% % \end{tcolorbox}
% % }



% \begin{document}





% \appendix
% \section{Related Works}
% In this section, we introduce related studies on similar tasks that might be confused with code optimization, as well as a number of related surveys that investigate topics similar to this study.
% % Before presenting LMs for code optimization, we first discuss prior studies on similar tasks that might be confused with code optimization, as well as a number of related surveys that investigate topics similar to this study. 

% \subsection{LM-related tasks}
% LMs have been employed for a number of code-related tasks, including code generation, refactoring and repair, and performance modeling, described as follows. 

% \textbf{LM-based code generation} translates a program specification into program code or executable binaries~\cite{coignion2024performance}. 
% For example, Li et al.~\cite{DBLP:journals/corr/abs-2203-07814} presented AlphaCode, a novel LM-based system for code generation that achieves competitive performance based on natural language programming problems. He et al.~\cite{he2024cocost} designed CoCoST to use LM in real-world programming scenarios by mimicking human coding processes, such as online searching and test case creation. Moreover, Liu et al.~\cite{liu2024evolution} introduced EoH, combining LMs and evolutionary computation methods for automatic algorithm design. 

% \textbf{LM-based code refactoring}, similar to code editing \cite{DBLP:conf/sigsoft/GuptaKBCGKRS023}, code rewriting \cite{cummins2024don} or code transformation \cite{palkowski2024gpt}, focuses on restructuring the design, structure, and components of code, without explicitly addressing performance metrics~\cite{cordeiro2024empirical}. For instance, Li et al.~\cite{li2023codeeditor} proposed CodeEditor, which generates code mutations from real-world code and learns to edit them back to the original, thereby capturing effective refactoring patterns. Cummins et al.~\cite{cummins2024don} emphasized generating refactoring transformations rather than directly rewriting code, allowing for easier inspection, debugging, and validation.

% Additionally, efforts have been focused on \textbf{LM-based code repair}, where LMs are used to identify and fix defects, bugs, or errors in code to restore its intended functionality and ensure correctness~\cite{zhang2024systematic}. As examples, Jin et al.~\cite{DBLP:conf/sigsoft/JinSTSLSS23} employed a retrieval-based prompt augmentation technique and task-oriented fine-tuning in InferFix, leveraging bug-type annotations and extended source code context to enhance bug detection and repair processes, and Zhang et al.~\cite{zhang2024autocoderover} leveraged code representation through abstract syntax trees (ASTs) and employs spectrum-based fault localization to generate effective patches, resolving software issues efficiently.

% Other works have targeted \textbf{LM-based code performance modeling}, which involves analyzing and understanding the performance characteristics of code, serving as a potential component of code optimization~\cite{chen2024reasoning}. Among others, Wang et al.~\cite{DBLP:journals/corr/abs-2406-12806} introduced PerfSense, which leverages LM agents and prompt chaining techniques to analyze source code and classify configurations as performance-sensitive or insensitive, thereby enhancing performance analysis.
% Besides, in the work by Nichols et al.~\cite{DBLP:journals/corr/abs-2306-17281}, an LM was fine-tuned on a curated dataset containing HPC and scientific codes, and is employed to predict the relative performance impact of changes made to the source code. 

% While the above studies are related to code optimization to some extent, they are not included in this survey because their primary focuses are different from our definition of code optimization\footnote{Note that although some studies do not explicitly define their task as code optimization, we have included them in this survey if in any steps the performance of existing code is improved, typical examples will be some studies for code editing, code refinement, and some code generation studies with iterative performance improvements.}. This survey aims to address this gap by focusing exclusively on the application of LMs for optimizing the performance of existing code or programs.

% \subsection{Related surveys}
% To the best of our knowledge, the most relevant surveys to ours are those focusing on \textbf{LMs for evolutionary algorithms (EAs)}, which involve solving optimization problems by iteratively improving a population of candidates through mechanisms inspired by biological evolution, such as selection, mutation, and crossover. Specifically, Huang et al.~\cite{huang2024large} discussed the roles of LMs in solving complex optimization problems through evolutionary mechanisms and provided future directions in this application, and Wu et al.~\cite{wu2024evolutionary} explored the collaborative strengths of LMs and EAs in three aspects: LM-enhanced EA, EA-enhanced LM, and their applications in optimization tasks. However, these surveys only cover a broad range of optimization problems, not specializing in enhancing the performance of existing programs.

% Besides, previous surveys have typically focused on \textbf{code optimization using traditional methods} involving compilers, machine learning (ML), and deep learning (DL) techniques~\cite{li2020deep, wang2018machine, bhatsurvey, wan2024deep, sun2024survey}. For instance, Wang et al.~\cite{wang2018machine} discussed the integration of ML into compiler optimization, highlighting its evolution over the past 50 years and its current status as a mainstream research area. More recently, Wan et al.~\cite{wan2024deep} conducted a comprehensive survey on deep learning for code intelligence, covering aspects such as code representations, DL techniques, application tasks, and public datasets.
% % ashouri2018survey, allamanis2018survey, ghaemi2024transformers

% Moreover, a few surveys have investigated the utilization of \textbf{LMs for code-related tasks}, including general code intelligence~\cite{DBLP:journals/corr/abs-2311-10372, DBLP:journals/entropy/WongGHHT23}, code generation~\cite{DBLP:journals/corr/abs-2406-00515, chen2024survey}, and code repair~\cite{zhang2024systematic}. In particular, Zhang et al.~\cite{zhang2023unifying} reviewed the evolution of LM-based techniques for code processing tasks from pre-trained Transformer to advanced retrieval and agentic approaches, and Chen et al.~\cite{chen2024survey} survey current methods and metrics for assessing code generation capabilities, identifying their limitations and proposing directions for future improvements.
% % zhang2023unifying, joel2024survey, DBLP:journals/corr/abs-2407-07064

% Additionally, there have been several surveys on the use of \textbf{LMs in general software engineering tasks}. For example, Hou et al.~\cite{hou2024largelanguagemodelssoftware} provided a comprehensive understanding of how LMs can optimize SE processes and outcomes, addressing gaps in existing research. Similarly, Fan et al.~\cite{DBLP:conf/fose-ws/FanGHLSYZ23} provided a comprehensive overview of the current state of research and future directions in LM-based software engineering, and Shi et al.~\cite{DBLP:journals/corr/abs-2404-04566} proposed a vision for the future of LLM4SE that includes a roadmap for research directions aimed at improving efficiency and reducing carbon emissions associated with LMs.

% % introduce why there is a knowledge gap for a survey specifically focus on LMs for code optimization
% Despite the existence of comprehensive surveys, there is a notable knowledge gap when it comes to a focused survey on the use of LMs specifically for code optimization. Therefore, this survey addresses this gap by systematically reviewing the current state of research and applications of LMs in code optimization, identifying the strengths and limitations of existing approaches, and providing guidance for future research directions.




% \bibliographystyle{plain}
% \bibliography{references}
% \end{document}

==> standalone_threats_to_validity.tex <==
% \documentclass[a4paper,10pt]{article}
% %\usepackage{pxfonts}
% \textwidth=148mm
% \textheight=250mm
% \voffset -25mm
% \hoffset -10mm
% \renewcommand{\baselinestretch}{1.1}
% \setlength{\parskip}{0.5\baselineskip}
% % \setlength\parindent{0pt}

% \usepackage{amsmath,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{booktabs}
% \usepackage{tikz,pgfplots}
% \usepackage{standalone}
% \usepackage[most]{tcolorbox}
% \usepackage{csquotes}
% \usepackage{url}
% \usepackage{multirow}
% \usetikzlibrary{arrows.meta}
% \usepackage{fancyhdr}
% \usepackage{threeparttable}
% \usepackage{subcaption}
% \usepackage{makecell}
% \usepackage{hyperref}
% \usepackage{newtxmath}
% \usepackage{pgf-pie}
% \usepackage{multirow}
% \usepackage{fontawesome5}
% \usepackage{pifont} % Provides check marks and crosses
% \usepackage{xspace}
% \usepackage{natbib}

% \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% % \newcommand{\keybox}[1]{
% % \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% % \em #1
% % \end{tcolorbox}
% % }

% \lstset{
%     language=Python,
%     basicstyle=\ttfamily\footnotesize,
%     keywordstyle=\color{blue},
%     stringstyle=\color{red},
%     commentstyle=\color{green},
%     morecomment=[l][\color{magenta}]{\#},
%     numbers=left,
%     numberstyle=\tiny\color{gray},
%     stepnumber=1,
%     numbersep=5pt,
%     showstringspaces=false,
%     breaklines=true,
%     frame=single,
%     backgroundcolor=\color{white},
%     captionpos=b
% }


% \makeatletter
% \tcbset{
%     myhbox/.style 2 args={%
%         enhanced, 
%         breakable,
%         colback=white,
%         colframe=cerublue!70,
%         attach boxed title to top left={yshift*=-\tcboxedtitleheight}, 
%         title={#2},
%         boxed title size=title,
%         boxed title style={%
%             sharp corners, 
%             rounded corners=northwest, 
%             colback=tcbcolframe, 
%             boxrule=0pt,
%         },
%         underlay boxed title={%
%             \path[fill=tcbcolframe] (title.south west)--(title.south east) 
%                 to[out=0, in=180] ([xshift=5mm]title.east)--
%                 (title.center-|frame.east)
%                 [rounded corners=\kvtcb@arc] |- 
%                 (frame.north) -| cycle; 
%         },
%         #1
%     }
% }   
% \makeatother

% \newtcolorbox{myhbox}[2][]{%
%     myhbox={#1}{#2}
% }

% \newcounter{findingcount}
% \setcounter{findingcount}{1} 
% \newcounter{suggestioncount}
% \setcounter{suggestioncount}{1}

% \newcommand{\keybox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=beaublue]
% \em #1
% \end{tcolorbox}
% }

% \newcommand{\suggestbox}[1]{
% \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=dollarbill!50]
% \em #1
% \end{tcolorbox}
% }
% % \usepackage{amsmath,amsfonts}
% % \usepackage{algorithmic}
% % \usepackage{graphicx}
% % \usepackage{textcomp}
% % \usepackage{xcolor}
% % \usepackage{booktabs}
% % \usepackage{tikz,pgfplots}
% % \usepackage{standalone}
% % \usepackage[most]{tcolorbox}
% % \usepackage{csquotes}
% % \usepackage{url}
% % \usepackage{multirow}
% % \usetikzlibrary{arrows.meta}
% % \usepackage{fancyhdr}
% % \usepackage{threeparttable}
% % \usepackage{subcaption}
% % \usepackage{makecell}
% % \usepackage{hyperref}
% % \usepackage{newtxmath}
% % \usepackage{pgf-pie}
% % \usepackage{multirow}
% % \usepackage{pifont} % Provides check marks and crosses
% % \usepackage{xspace}
% % \usepackage{natbib}

% % \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
% % \definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
% % \definecolor{dollarbill}{rgb}{0.52, 0.73, 0.4}
% % \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% % \definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
% % \definecolor{cerublue}{rgb}{0.16, 0.32, 0.75}
% % \definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
% % \definecolor{iceberg}{rgb}{0.44, 0.65, 0.82}


% % \newcommand{\cmark}{\textcolor{applegreen}{\ding{51}}} % Green check mark
% % \newcommand{\xmark}{\textcolor{amaranth}{\ding{55}}} % Red cross mark

% % \newcommand\FIXME[1]{{\color{red}#1}\xspace}

% % \newcommand{\keybox}[1]{
% % \begin{tcolorbox}[leftrule=1mm,toprule=0mm,bottomrule=0mm,left=1pt,right=2pt,top=2pt,bottom=2pt, colback=cerublue!40]
% % \em #1
% % \end{tcolorbox}
% % }



% \begin{document}





% \appendix
% \section{Threats to Validity}
% \label{sec:threats_to_validity}

% Our survey was conducted according to well-established literature review guidelines for systematic literature reviews (SLRs) in software engineering (SE)~\cite{keele2007guidelines}. Naturally, as with many other SLRs, our survey has room for improvement. We discuss a few points below. 

% \subsection{Search Strategy Threats} 
% Threats to the search strategy can occur if our search methods do not cover enough relevant studies. To mitigate this, we employed a systematic search strategy~\cite{DBLP:journals/corr/Gong24Deep, hou2024largelanguagemodelssoftware} across multiple databases. We carefully refined the search string using the QGS~\cite{DBLP:journals/infsof/ZhangBT11} to ensure a wide and accurate coverage of relevant studies. Additionally, we performed a comprehensive snowballing search to identify any significant studies that may have been missed. 

% \subsection{Study Selection Threats} 
% Threats to study selection arise when the inclusion and exclusion criteria are not properly designed, potentially leading to biased results. To address this, we defined clear and precise inclusion and exclusion criteria before the selection process. Multiple researchers independently screened the studies, and any discrepancies were resolved through discussion or consulting a third party, ensuring a balanced and unbiased selection of studies. Furthermore, with the merging trend of LMs, most primary studies are from arXiv and are not peer-reviewed, posing a validity threat. To handle this, we conducted rigorous study quality assessments using specialized quality assessment criteria (QAC) to filter out low-quality studies~\cite{hou2024largelanguagemodelssoftware, DBLP:journals/tse/WangHGGZFSLZN23}.

% \subsection{Data Collection Threats} 
% Threats to data collection can affect the validity of our findings if the data extraction process is flawed or subjective. To mitigate this, we developed a standardized table to record all data collected in this process, and any modifications to the table were independently reviewed by at least two researchers to verify the accuracy of the extracted data~\cite{DBLP:journals/corr/Gong24Deep}. Any inconsistencies were discussed and resolved collaboratively to maintain data integrity.

% By addressing these potential threats to validity, we aim to enhance the robustness and reliability of our survey findings.




% \bibliographystyle{plain}
% \bibliography{references}
% \end{document}

==> threats_to_validity.tex <==
\section{Threats to Validity}
\label{sec:threats_to_validity}

Our survey was conducted according to well-established literature review guidelines for SLR in SE~\cite{keele2007guidelines}. Naturally, as with many other SLRs, our survey has room for improvement. We discussed a few points here. 

% \subsection{Search Strategy Threats} 
\textbf{Search strategy threats} can occur if our search methods do not cover enough relevant studies. To mitigate this, we employed a systematic search strategy~\cite{DBLP:journals/corr/Gong24Deep, hou2024largelanguagemodelssoftware} across multiple databases. We carefully refined the search string using the QGS~\cite{DBLP:journals/infsof/ZhangBT11} to ensure a wide and accurate coverage of relevant studies. Additionally, we performed a comprehensive snowballing search to identify any significant studies that may have been missed. 

% \subsection{Study Selection Threats} 
\textbf{Study selection threats} arise when the inclusion and exclusion criteria are not properly designed, potentially leading to biased results. To address this, we defined clear and precise inclusion and exclusion criteria before the selection process. Multiple researchers independently screened the studies, and any discrepancies were resolved through discussion or consulting a third party, ensuring a balanced and unbiased selection of studies. Furthermore, with the merging trend of LMs, most primary studies are from arXiv and are not peer reviewed, posing a validity threat. To handle this, we conducted rigorous study quality assessments using specified QACs in Table~\ref{tb:quality_assessment} to filter out low-quality studies~\cite{hou2024largelanguagemodelssoftware, DBLP:journals/tse/WangHGGZFSLZN23}.

% \subsection{Data Collection Threats} 
\textbf{Data collection threats} can affect the validity of our findings if the data extraction process is flawed or subjective. To mitigate this, we developed a standardized table to record all data collected in this process, and any modification to the table should be independently reviewed by at least two researchers to verify the accuracy of the extracted data~\cite{DBLP:journals/corr/Gong24Deep}. Any inconsistencies were discussed and resolved collaboratively to maintain data integrity.

By addressing these potential threats to validity, we aim to enhance the robustness and reliability of our survey findings.
